Questions of minimality for DDMOGs and cycle ornaments

Difference distance magic oriented graphs (DDMOGs) are oriented graphs whose vertices admit a bijective labeling by consecutive positive integers such that every vertex has weight zero, where the weight is the sum of the labels of its in-neighbors minus the sum of the labels of its out-neighbors. We investigate minimality and sparsity questions for DDMOGs and their ornaments. First, we develop new constructions of cycle-based ornaments that reduce the number of cycles required for a given number of attachment nodes and identify minimal cycle lengths in several cases. Second, we determine the minimum number of arcs in a nontrivial DDMOG of order $n$, combining computational enumeration for small orders with theoretical lower bounds and constructions. Langford sequences provide a key tool in these constructions, enabling us to partition consecutive labels into difference triples and thereby construct sparse DDMOGs. Finally, we use related constructions to obtain generalized ornaments with no internal arcs. These results advance the study of minimal constructions in difference distance magic labeling and provide new methods for building sparse DDMOGs.

==> tables/order-10-even-labelings.tex <==
\begin{tabular}{| c | c |}
\hline
\(n\) and \(x\) & Base Labeling and Difference Triples\\
\hline
\(n=22\) & 
7,4,10,12,5,16,1,8,17,11\\
\cline{2-2}
\(x=2\)
&(15,3,18),(9,13,22),(19,2,21),(6,14,20)\\
\hline 
\(n=34\) & 
17,16,20,8,14,24,1,18,22,21\\
\cline{2-2}
\(x=4\)
&(9,10,19),(12,11,23),(5,25,30),(2,13,15),(27,4,31),(7,26,33),(6,28,34),(29,3,32)\\
\hline 
\(n=46\) & 
36,18,17,27,13,45,8,44,40,25\\
\cline{2-2}
\(x=6\)
&(21,10,31),(12,11,23),(20,2,22),(15,9,24),(14,19,33),(28,7,35),(32,6,38),(34,5,39),\\
&(37,4,41),(29,1,30),(3,43,46),(26,16,42)\\
\hline 
\(n=58\) & 
13,12,20,44,14,56,15,28,58,35\\
\cline{2-2}
\(x=8\)
&(33,10,43),(4,22,26),(2,52,54),(31,24,55),(6,36,42),(1,29,30),(23,17,40),(16,21,37),\\
&(5,41,46),(25,7,32),(11,39,50),(27,18,45),(38,9,47),(3,48,51),(8,49,57),(19,34,53)\\
\hline 
\(n=70\) & 
25,65,34,2,64,67,17,42,66,51\\
\cline{2-2}
\(x=10\)
&(1,11,12),(29,7,36),(19,33,52),(45,4,49),(44,18,62),(32,28,60),(37,20,57),(38,21,59),\\
&(3,47,50),(53,16,69),(24,6,30),(43,15,58),(8,46,54),(14,56,70),(5,22,27),(39,9,48),\\
&(10,31,41),(40,23,63),(35,26,61),(55,13,68)\\
\hline 
\(n=82\) & 
52,69,65,2,58,71,15,67,60,80\\
\cline{2-2}
\(x=12\)
&(9,11,20),(44,33,77),(56,10,66),(21,16,37),(5,26,31),(47,6,53),(14,41,55),(43,35,78),\\
&(25,50,75),(1,73,74),(4,72,76),(18,63,81),(23,36,59),(12,70,82),(24,8,32),(30,49,79),\\
&(54,3,57),(42,22,64),(39,7,46),(17,45,62),(19,29,48),(27,34,61),(38,13,51),(40,28,68)\\
\hline 
\(n=94\) & 
88,73,44,3,59,76,6,94,62,50\\
\cline{2-2}
\(x=14\)
&(42,47,89),(38,39,77),(49,7,56),(31,32,63),(26,14,40),(10,71,81),(9,78,87),(20,33,53),\\
&(22,29,51),(1,91,92),(30,55,85),(21,24,45),(37,46,83),(17,58,75),(11,82,93),(16,74,90),\\
&(41,23,64),(35,34,69),(36,18,54),(67,5,72),(52,28,80),(57,8,65),(19,60,79),(43,25,68),\\
&(13,48,61),(12,15,27),(66,4,70),(84,2,86)\\
\hline 
\(n=106\) & 
29,83,22,3,9,86,56,85,12,78\\
\cline{2-2}
\(x=16\)
&(24,65,89),(18,63,81),(1,4,5),(49,55,104),(52,51,103),(15,67,82),(68,2,70),(69,27,96),\\
&(11,8,19),(14,66,80),(47,45,92),(53,48,101),(34,57,91),(25,73,98),(72,7,79),(21,84,105),\\
&(59,40,99),(31,75,106),(43,50,93),(37,60,97),(23,64,87),(62,32,94),(39,61,100),(10,6,16),\\
&(71,17,88),(36,38,74),(20,13,33),(28,30,58),(76,26,102),(46,44,90),(42,35,77),(54,41,95)\\
\hline 
\(n=118\) & 
39,51,34,24,40,75,77,116,64,111\\
\cline{2-2}
\(x=18\)
&(31,41,72),(16,21,37),(5,93,98),(108,1,109),(49,30,79),(52,28,80),(54,29,83),(55,26,81),\\
&(18,45,63),(33,43,76),(60,25,85),(35,38,73),(59,27,86),(62,22,84),(71,36,107),(96,4,100),\\
&(15,53,68),(69,19,88),(47,50,97),(70,20,90),(74,17,91),(102,3,105),(82,12,94),(13,99,112),\\
&(92,11,103),(106,9,115),(104,10,114),(23,44,67),(87,2,89),(32,46,78),(42,14,56),(110,7,117),\\
&(65,48,113),(95,6,101),(8,58,66),(57,61,118)\\
\hline 
\(n=130\) & 
10,58,5,8,12,66,69,79,20,74\\
\cline{2-2}
\(x=20\)
&(92,38,130),(81,40,121),(34,28,62),(95,32,127),(101,1,102),(117,9,126),(4,84,88),(60,23,83),\\
&(51,52,103),(61,53,114),(29,77,106),(47,82,129),(76,14,90),(16,100,116),(55,57,112),(3,119,122),\\
&(63,26,89),(18,93,111),(71,25,96),(35,80,115),(11,30,41),(46,64,110),(43,44,87),(6,85,91),\\
&(65,2,67),(75,33,108),(15,7,22),(42,56,98),(21,97,118),(13,36,49),(31,94,125),(24,99,123),\\
&(107,17,124),(54,19,73),(37,68,105),(78,50,128),(48,72,120),(27,86,113),(59,45,104),(70,39,109)\\
\hline 
\end{tabular}

==> tables/order-10-odd-labelings.tex <==
\begin{tabular}{| c | c |}
\hline
\(n\) and \(x\) & Base Labeling and Difference Triples\\
\hline
\(n=19\) & 
11,10,2,1,12,6,17,3,8,13,18,4,15\\
\cline{2-2}
\(x=1\)
&(9,7,16),(5,14,19)\\
\hline 
\(n=31\) & 
27,12,16,1,28,2,29,3,18,15,30,4,31\\
\cline{2-2}
\(x=3\)
&(13,10,23),(14,8,22),(9,11,20),(17,7,24),(19,6,25),(21,5,26)\\
\hline 
\(n=43\) & 
6,4,20,18,24,5,11,3,25,7,29,21,27\\
\cline{2-2}
\(x=5\)
&(22,17,39),(15,16,31),(8,35,43),(9,28,37),(12,26,38),(13,23,36),(10,30,40),(1,41,42),\\
&(19,14,33),(2,32,34)\\
\hline 
\(n=55\) & 
12,32,10,30,42,13,25,4,23,36,55,34,46\\
\cline{2-2}
\(x=7\)
&(16,28,44),(3,15,18),(52,1,53),(5,19,24),(26,22,48),(9,45,54),(2,35,37),(27,6,33),\\
&(41,8,49),(17,21,38),(29,14,43),(39,11,50),(20,31,51),(7,40,47)\\
\hline 
\(n=67\) & 
21,37,3,19,40,25,46,26,28,63,65,45,66\\
\cline{2-2}
\(x=9\)
&(49,15,64),(22,32,54),(8,50,58),(13,42,55),(9,35,44),(27,29,56),(1,30,31),(2,5,7),\\
&(6,53,59),(43,17,60),(47,14,61),(12,11,23),(20,16,36),(18,39,57),(48,4,52),(33,34,67),\\
&(41,10,51),(38,24,62)\\
\hline 
\(n=79\) & 
1,35,7,41,42,23,24,33,30,68,65,74,75\\
\cline{2-2}
\(x=11\)
&(58,21,79),(16,60,76),(4,22,26),(11,55,66),(2,61,63),(20,50,70),(9,38,47),(52,17,69),\\
&(18,39,57),(27,37,64),(28,34,62),(14,53,67),(29,44,73),(12,31,43),(8,48,56),(46,25,71),\\
&(32,45,77),(51,3,54),(36,13,49),(6,72,78),(10,5,15),(40,19,59)\\
\hline 
\(n=91\) & 
25,46,16,37,62,3,28,15,19,61,65,52,77\\
\cline{2-2}
\(x=13\)
&(32,43,75),(33,50,83),(6,4,10),(1,20,21),(8,63,71),(23,44,67),(5,53,58),(31,29,60),\\
&(27,55,82),(22,34,56),(51,35,86),(2,66,68),(36,9,45),(57,30,87),(14,76,90),(49,40,89),\\
&(42,39,81),(69,11,80),(13,59,72),(84,7,91),(38,41,79),(48,26,74),(17,47,64),(12,73,85),\\
&(24,54,78),(18,70,88)\\
\hline 
\(n=103\) & 
22,14,56,48,70,12,34,6,68,20,82,54,76\\
\cline{2-2}
\(x=15\)
&(10,67,77),(31,35,66),(3,100,103),(27,42,69),(32,17,49),(30,29,59),(7,91,98),(60,1,61),\\
&(33,25,58),(41,23,64),(28,51,79),(24,57,81),(5,90,95),(16,71,87),(2,72,74),(83,9,92),\\
&(46,43,89),(38,37,75),(36,52,88),(50,47,97),(55,18,73),(86,13,99),(85,11,96),(21,44,65),\\
&(53,40,93),(15,63,78),(94,8,102),(80,4,84),(19,26,45),(62,39,101)\\
\hline 
\(n=115\) & 
86,94,2,10,96,17,103,16,19,110,113,26,112\\
\cline{2-2}
\(x=17\)
&(69,30,99),(54,44,98),(70,41,111),(11,84,95),(47,40,87),(35,62,97),(39,63,102),(43,31,74),\\
&(21,6,27),(9,42,51),(14,101,115),(5,67,72),(55,13,68),(76,29,105),(64,1,65),(32,45,77),\\
&(59,33,92),(22,53,75),(8,12,20),(57,23,80),(37,36,73),(50,58,108),(88,3,91),(7,93,100),\\
&(60,46,106),(56,15,71),(81,28,109),(4,78,82),(52,38,90),(48,66,114),(79,25,104),(89,18,107),\\
&(34,49,83),(24,61,85)\\
\hline 
\(n=127\) & 
60,68,20,28,88,11,71,26,31,94,99,54,114\\
\cline{2-2}
\(x=19\)
&(15,18,33),(45,39,84),(89,1,90),(119,2,121),(43,40,83),(44,14,58),(47,65,112),(13,100,113),\\
&(32,24,56),(50,77,127),(57,61,118),(10,107,117),(87,5,92),(78,42,120),(27,79,106),(53,51,104),\\
&(7,96,103),(30,55,85),(41,81,122),(62,36,98),(9,93,102),(76,21,97),(73,35,108),(34,91,125),\\
&(17,8,25),(37,74,111),(75,49,124),(110,6,116),(59,64,123),(67,38,105),(22,48,70),(12,4,16),\\
&(3,69,72),(66,29,95),(82,19,101),(46,80,126),(23,86,109),(52,63,115)\\
\hline 
\end{tabular}

==> tables/order-13-even-labelings.tex <==
\begin{tabular}{| c | c |}
\hline
\(n\) and \(x\) & Base Labeling and Difference Triples\\
\hline
\(n=25\) & 
17,12,7,2,19,1,18,4,8,16,20,6,23\\
\cline{2-2}
\(x=2\)
&(13,9,22),(11,14,25),(10,5,15),(21,3,24)\\
\hline 
\(n=37\) & 
15,8,19,12,27,9,24,10,28,18,36,22,37\\
\cline{2-2}
\(x=4\)
&(14,20,34),(2,23,25),(6,5,11),(4,17,21),(30,1,31),(7,26,33),(16,13,29),(32,3,35)\\
\hline 
\(n=49\) & 
27,20,19,12,39,2,29,3,21,23,41,15,42\\
\cline{2-2}
\(x=6\)
&(31,5,36),(38,7,45),(9,28,37),(33,16,49),(44,4,48),(8,22,30),(34,6,40),(10,25,35),\\
&(11,13,24),(26,17,43),(14,18,32),(46,1,47)\\
\hline 
\(n=61\) & 
15,3,24,12,27,21,36,31,45,34,48,43,58\\
\cline{2-2}
\(x=8\)
&(47,10,57),(8,42,50),(32,6,38),(19,41,60),(13,17,30),(16,37,53),(35,26,61),(18,22,40),\\
&(49,5,54),(2,44,46),(9,11,20),(28,1,29),(25,14,39),(7,52,59),(33,23,56),(4,51,55)\\
\hline 
\(n=73\) & 
61,20,43,2,63,4,65,3,47,23,67,5,66\\
\cline{2-2}
\(x=10\)
&(33,35,68),(6,11,17),(15,27,42),(24,16,40),(1,72,73),(31,21,52),(9,46,55),(44,14,58),\\
&(29,22,51),(38,12,50),(53,7,60),(25,39,64),(28,41,69),(13,57,70),(34,37,71),(10,49,59),\\
&(30,32,62),(8,48,56),(26,19,45),(18,36,54)\\
\hline 
\(n=85\) & 
17,37,16,36,53,18,35,19,34,56,71,55,72\\
\cline{2-2}
\(x=12\)
&(44,41,85),(45,4,49),(64,12,76),(32,46,78),(60,14,74),(9,29,38),(30,31,61),(2,81,83),\\
&(70,7,77),(58,8,66),(10,33,43),(39,24,63),(25,15,40),(62,11,73),(57,27,84),(13,67,80),\\
&(51,1,52),(22,28,50),(21,26,47),(42,23,65),(20,48,68),(69,6,75),(5,54,59),(79,3,82)\\
\hline 
\(n=97\) & 
6,9,46,49,55,35,41,42,81,51,90,91,97\\
\cline{2-2}
\(x=14\)
&(1,3,4),(21,58,79),(36,34,70),(65,13,78),(45,27,72),(20,28,48),(68,19,87),(63,29,92),\\
&(18,62,80),(22,61,83),(32,25,57),(14,71,85),(5,10,15),(26,56,82),(16,38,54),(24,53,77),\\
&(37,47,84),(44,50,94),(17,59,76),(93,2,95),(60,7,67),(31,43,74),(75,11,86),(88,8,96),\\
&(66,23,89),(12,52,64),(30,39,69),(40,33,73)\\
\hline 
\(n=109\) & 
31,24,29,22,53,44,75,36,73,60,97,58,89\\
\cline{2-2}
\(x=16\)
&(26,41,67),(20,35,55),(10,98,108),(8,32,40),(69,30,99),(71,23,94),(37,63,100),(43,27,70),\\
&(49,57,106),(25,34,59),(62,21,83),(66,19,85),(72,16,88),(68,13,81),(102,2,104),(76,14,90),\\
&(86,9,95),(12,52,64),(45,46,91),(33,15,48),(18,56,74),(78,6,84),(38,1,39),(65,17,82),\\
&(3,77,80),(87,5,92),(11,50,61),(54,47,101),(105,4,109),(96,7,103),(51,42,93),(79,28,107)\\
\hline 
\(n=121\) & 
36,75,2,41,77,14,50,42,16,117,91,83,119\\
\cline{2-2}
\(x=18\)
&(39,58,97),(3,115,118),(46,55,101),(61,47,108),(30,81,111),(78,18,96),(64,7,71),(45,43,88),\\
&(59,9,68),(33,80,113),(26,56,82),(15,90,105),(35,28,63),(6,70,76),(8,40,48),(13,86,99),\\
&(17,92,109),(65,1,66),(38,22,60),(73,34,107),(74,24,98),(10,84,94),(53,57,110),(12,20,32),\\
&(72,31,103),(79,23,102),(37,67,104),(19,25,44),(100,21,121),(49,5,54),(85,27,112),(51,69,120),\\
&(87,29,116),(52,62,114),(89,4,93),(11,95,106)\\
\hline 
\(n=133\) & 
2,24,49,71,73,28,30,51,77,75,101,122,124\\
\cline{2-2}
\(x=20\)
&(36,76,112),(45,84,129),(6,103,109),(60,48,108),(12,93,105),(52,62,114),(8,96,104),(47,66,113),\\
&(67,11,78),(64,21,85),(57,54,111),(23,92,115),(58,69,127),(7,3,10),(80,39,119),(79,42,121),\\
&(46,61,107),(29,89,118),(20,86,106),(82,17,99),(38,50,88),(40,32,72),(59,35,94),(83,14,97),\\
&(43,74,117),(110,15,125),(34,98,132),(44,87,131),(19,22,41),(16,65,81),(18,9,27),(4,126,130),\\
&(1,90,91),(37,33,70),(25,31,56),(95,5,100),(120,13,133),(102,26,128),(55,68,123),(53,63,116)\\
\hline 
\end{tabular}

==> tables/order-13-odd-labelings.tex <==
\begin{tabular}{| c | c |}
\hline
\(n\) and \(x\) & Base Labeling and Difference Triples\\
\hline
\(n=19\) & 
11,10,2,1,12,6,17,3,8,13,18,4,15\\
\cline{2-2}
\(x=1\)
&(9,7,16),(5,14,19)\\
\hline 
\(n=31\) & 
27,12,16,1,28,2,29,3,18,15,30,4,31\\
\cline{2-2}
\(x=3\)
&(13,10,23),(14,8,22),(9,11,20),(17,7,24),(19,6,25),(21,5,26)\\
\hline 
\(n=43\) & 
6,4,20,18,24,5,11,3,25,7,29,21,27\\
\cline{2-2}
\(x=5\)
&(22,17,39),(15,16,31),(8,35,43),(9,28,37),(12,26,38),(13,23,36),(10,30,40),(1,41,42),\\
&(19,14,33),(2,32,34)\\
\hline 
\(n=55\) & 
12,32,10,30,42,13,25,4,23,36,55,34,46\\
\cline{2-2}
\(x=7\)
&(16,28,44),(3,15,18),(52,1,53),(5,19,24),(26,22,48),(9,45,54),(2,35,37),(27,6,33),\\
&(41,8,49),(17,21,38),(29,14,43),(39,11,50),(20,31,51),(7,40,47)\\
\hline 
\(n=67\) & 
21,37,3,19,40,25,46,26,28,63,65,45,66\\
\cline{2-2}
\(x=9\)
&(49,15,64),(22,32,54),(8,50,58),(13,42,55),(9,35,44),(27,29,56),(1,30,31),(2,5,7),\\
&(6,53,59),(43,17,60),(47,14,61),(12,11,23),(20,16,36),(18,39,57),(48,4,52),(33,34,67),\\
&(41,10,51),(38,24,62)\\
\hline 
\(n=79\) & 
1,35,7,41,42,23,24,33,30,68,65,74,75\\
\cline{2-2}
\(x=11\)
&(58,21,79),(16,60,76),(4,22,26),(11,55,66),(2,61,63),(20,50,70),(9,38,47),(52,17,69),\\
&(18,39,57),(27,37,64),(28,34,62),(14,53,67),(29,44,73),(12,31,43),(8,48,56),(46,25,71),\\
&(32,45,77),(51,3,54),(36,13,49),(6,72,78),(10,5,15),(40,19,59)\\
\hline 
\(n=91\) & 
25,46,16,37,62,3,28,15,19,61,65,52,77\\
\cline{2-2}
\(x=13\)
&(32,43,75),(33,50,83),(6,4,10),(1,20,21),(8,63,71),(23,44,67),(5,53,58),(31,29,60),\\
&(27,55,82),(22,34,56),(51,35,86),(2,66,68),(36,9,45),(57,30,87),(14,76,90),(49,40,89),\\
&(42,39,81),(69,11,80),(13,59,72),(84,7,91),(38,41,79),(48,26,74),(17,47,64),(12,73,85),\\
&(24,54,78),(18,70,88)\\
\hline 
\(n=103\) & 
22,14,56,48,70,12,34,6,68,20,82,54,76\\
\cline{2-2}
\(x=15\)
&(10,67,77),(31,35,66),(3,100,103),(27,42,69),(32,17,49),(30,29,59),(7,91,98),(60,1,61),\\
&(33,25,58),(41,23,64),(28,51,79),(24,57,81),(5,90,95),(16,71,87),(2,72,74),(83,9,92),\\
&(46,43,89),(38,37,75),(36,52,88),(50,47,97),(55,18,73),(86,13,99),(85,11,96),(21,44,65),\\
&(53,40,93),(15,63,78),(94,8,102),(80,4,84),(19,26,45),(62,39,101)\\
\hline 
\(n=115\) & 
86,94,2,10,96,17,103,16,19,110,113,26,112\\
\cline{2-2}
\(x=17\)
&(69,30,99),(54,44,98),(70,41,111),(11,84,95),(47,40,87),(35,62,97),(39,63,102),(43,31,74),\\
&(21,6,27),(9,42,51),(14,101,115),(5,67,72),(55,13,68),(76,29,105),(64,1,65),(32,45,77),\\
&(59,33,92),(22,53,75),(8,12,20),(57,23,80),(37,36,73),(50,58,108),(88,3,91),(7,93,100),\\
&(60,46,106),(56,15,71),(81,28,109),(4,78,82),(52,38,90),(48,66,114),(79,25,104),(89,18,107),\\
&(34,49,83),(24,61,85)\\
\hline 
\(n=127\) & 
60,68,20,28,88,11,71,26,31,94,99,54,114\\
\cline{2-2}
\(x=19\)
&(15,18,33),(45,39,84),(89,1,90),(119,2,121),(43,40,83),(44,14,58),(47,65,112),(13,100,113),\\
&(32,24,56),(50,77,127),(57,61,118),(10,107,117),(87,5,92),(78,42,120),(27,79,106),(53,51,104),\\
&(7,96,103),(30,55,85),(41,81,122),(62,36,98),(9,93,102),(76,21,97),(73,35,108),(34,91,125),\\
&(17,8,25),(37,74,111),(75,49,124),(110,6,116),(59,64,123),(67,38,105),(22,48,70),(12,4,16),\\
&(3,69,72),(66,29,95),(82,19,101),(46,80,126),(23,86,109),(52,63,115)\\
\hline 
\end{tabular}

==> tables/order-14-even-labelings.tex <==
\begin{tabular}{| c | c |}
\hline
\(n\) and \(x\) & Base Labeling and Difference Triples\\
\hline
\(n=26\) & 
11,5,20,10,15,17,1,22,25,21,7,18,12,23\\
\cline{2-2}
\(x=2\)
&(24,2,26),(9,4,13),(8,6,14),(16,3,19)\\
\hline 
\(n=38\) & 
21,4,2,13,14,33,22,37,27,24,5,26,9,30\\
\cline{2-2}
\(x=4\)
&(12,16,28),(15,8,23),(7,25,32),(18,20,38),(10,1,11),(31,3,34),(6,29,35),(17,19,36)\\
\hline 
\(n=50\) & 
13,19,23,28,5,17,9,36,33,32,16,29,35,48\\
\cline{2-2}
\(x=6\)
&(6,8,14),(25,21,46),(12,10,22),(30,20,50),(34,15,49),(24,7,31),(41,3,44),(40,2,42),\\
&(38,1,39),(26,11,37),(4,43,47),(18,27,45)\\
\hline 
\(n=62\) & 
21,2,23,27,9,54,15,56,36,38,8,29,10,31\\
\cline{2-2}
\(x=8\)
&(43,3,46),(28,24,52),(4,18,22),(20,19,39),(33,14,47),(35,13,48),(37,12,49),(40,1,41),\\
&(34,11,45),(42,16,58),(44,17,61),(50,7,57),(53,6,59),(55,5,60),(26,25,51),(32,30,62)\\
\hline 
\(n=74\) & 
9,12,64,31,42,13,1,25,73,65,2,11,14,23\\
\cline{2-2}
\(x=10\)
&(24,22,46),(7,49,56),(33,36,69),(40,21,61),(43,20,63),(37,18,55),(26,4,30),(27,44,71),\\
&(32,16,48),(39,35,74),(53,15,68),(6,52,58),(34,38,72),(62,5,67),(47,19,66),(10,50,60),\\
&(17,28,45),(29,41,70),(54,3,57),(51,8,59)\\
\hline 
\(n=86\) & 
31,22,50,72,12,41,19,63,84,69,20,51,42,73\\
\cline{2-2}
\(x=12\)
&(48,27,75),(78,5,83),(32,53,85),(55,4,59),(45,2,47),(10,66,76),(39,25,64),(54,23,77),\\
&(16,46,62),(1,7,8),(36,29,65),(52,15,67),(26,18,44),(61,13,74),(6,11,17),(34,24,58),\\
&(30,56,86),(70,9,79),(33,49,82),(3,35,38),(28,40,68),(43,37,80),(21,60,81),(57,14,71)\\
\hline 
\(n=98\) & 
19,2,37,3,65,9,52,11,68,89,61,80,63,82\\
\cline{2-2}
\(x=14\)
&(85,12,97),(5,29,34),(58,18,76),(24,35,59),(15,25,40),(43,55,98),(21,67,88),(6,69,75),\\
&(54,16,70),(53,39,92),(44,42,86),(48,36,84),(50,46,96),(14,57,71),(45,38,83),(4,91,95),\\
&(17,64,81),(23,56,79),(13,20,33),(32,28,60),(27,66,93),(41,49,90),(73,1,74),(31,47,78),\\
&(7,87,94),(10,62,72),(8,22,30),(26,51,77)\\
\hline 
\(n=110\) & 
53,19,72,3,23,77,37,96,26,109,14,67,33,86\\
\cline{2-2}
\(x=16\)
&(79,5,84),(10,61,71),(11,46,57),(70,24,94),(13,39,52),(51,30,81),(49,56,105),(6,16,22),\\
&(18,42,60),(59,31,90),(12,88,100),(43,55,98),(25,41,66),(40,8,48),(95,4,99),(9,80,89),\\
&(27,64,91),(38,36,74),(85,21,106),(34,68,102),(28,75,103),(47,54,101),(50,58,108),(1,92,93),\\
&(32,78,110),(82,15,97),(2,63,65),(35,69,104),(29,44,73),(87,20,107),(76,7,83),(45,17,62)\\
\hline 
\(n=122\) & 
59,3,51,32,29,53,47,56,61,98,38,97,41,100\\
\cline{2-2}
\(x=18\)
&(91,20,111),(54,62,116),(103,15,118),(44,69,113),(63,5,68),(18,27,45),(26,13,39),(24,81,105),\\
&(86,4,90),(36,46,82),(2,93,95),(52,65,117),(23,55,78),(75,40,115),(96,25,121),(84,28,112),\\
&(80,22,102),(50,72,122),(7,85,92),(48,19,67),(73,34,107),(94,14,108),(16,88,104),(8,101,109),\\
&(30,57,87),(49,71,120),(64,42,106),(58,12,70),(9,74,83),(21,89,110),(10,1,11),(31,6,37),\\
&(17,60,77),(43,76,119),(66,33,99),(35,79,114)\\
\hline 
\(n=134\) & 
33,50,14,16,57,80,18,130,73,32,25,58,75,108\\
\cline{2-2}
\(x=20\)
&(13,77,90),(27,78,105),(52,69,121),(37,91,128),(89,11,100),(51,45,96),(2,124,126),(3,101,104),\\
&(26,87,113),(6,76,82),(66,68,134),(23,30,53),(95,36,131),(24,92,116),(56,29,85),(46,35,81),\\
&(40,39,79),(19,67,86),(112,10,122),(43,1,44),(60,28,88),(17,115,132),(64,47,111),(8,98,106),\\
&(107,20,127),(97,22,119),(70,48,118),(4,110,114),(84,9,93),(55,65,120),(42,41,83),(21,102,123),\\
&(94,5,99),(74,59,133),(12,117,129),(71,38,109),(54,7,61),(15,34,49),(62,63,125),(31,72,103)\\
\hline 
\end{tabular}

==> tables/order-15-even-labelings.tex <==
\begin{tabular}{| c | c |}
\hline
\(n\) and \(x\) & Base Labeling and Difference Triples\\
\hline
\(n=27\) & 
2,8,9,11,5,4,6,14,16,15,18,19,26,27,20\\
\cline{2-2}
\(x=2\)
&(10,7,17),(12,13,25),(21,3,24),(22,1,23)\\
\hline 
\(n=39\) & 
2,16,28,30,1,6,8,29,31,36,11,19,27,35,37\\
\cline{2-2}
\(x=4\)
&(3,18,21),(7,32,39),(12,5,17),(14,10,24),(4,22,26),(23,15,38),(20,13,33),(9,25,34)\\
\hline 
\(n=51\) & 
18,20,9,27,7,4,22,16,34,31,10,13,30,33,38\\
\cline{2-2}
\(x=6\)
&(17,19,36),(6,39,45),(21,8,29),(25,26,51),(11,37,48),(28,15,43),(1,23,24),(32,12,44),\\
&(2,40,42),(5,41,46),(14,35,49),(3,47,50)\\
\hline 
\(n=63\) & 
6,2,8,14,12,37,43,20,26,51,34,56,36,58,63\\
\cline{2-2}
\(x=8\)
&(21,19,40),(1,60,61),(13,42,55),(32,30,62),(11,28,39),(22,25,47),(24,33,57),(5,4,9),\\
&(17,27,44),(49,3,52),(16,29,45),(38,10,48),(41,18,59),(31,23,54),(46,7,53),(35,15,50)\\
\hline 
\(n=75\) & 
15,8,17,32,26,7,22,43,58,39,60,37,68,45,65\\
\cline{2-2}
\(x=10\)
&(30,34,64),(21,51,72),(25,41,66),(50,2,52),(47,14,61),(23,44,67),(53,3,56),(10,9,19),\\
&(29,28,57),(5,69,74),(48,11,59),(54,1,55),(12,6,18),(46,24,70),(40,35,75),(4,16,20),\\
&(27,36,63),(33,38,71),(42,31,73),(13,49,62)\\
\hline 
\(n=87\) & 
57,24,11,68,7,6,63,18,75,74,41,34,65,58,81\\
\cline{2-2}
\(x=12\)
&(83,3,86),(5,40,45),(43,33,76),(50,32,82),(20,22,42),(12,48,60),(2,77,79),(53,27,80),\\
&(39,23,62),(55,16,71),(9,26,35),(38,8,46),(17,13,30),(66,1,67),(59,10,69),(36,25,61),\\
&(15,37,52),(47,4,51),(49,29,78),(70,14,84),(56,31,87),(19,54,73),(21,64,85),(28,44,72)\\
\hline 
\(n=99\) & 
7,28,24,31,18,27,34,42,49,58,44,45,72,73,76\\
\cline{2-2}
\(x=14\)
&(40,52,92),(62,35,97),(71,25,96),(22,48,70),(78,12,90),(9,89,98),(59,1,60),(3,63,66),\\
&(93,2,95),(17,57,74),(6,85,91),(21,33,54),(32,55,87),(5,10,15),(20,61,81),(50,29,79),\\
&(68,16,84),(83,11,94),(36,39,75),(37,14,51),(46,19,65),(41,47,88),(26,38,64),(8,69,77),\\
&(30,23,53),(13,67,80),(43,56,99),(4,82,86)\\
\hline 
\(n=111\) & 
1,8,5,6,12,49,50,17,18,55,75,94,83,102,67\\
\cline{2-2}
\(x=16\)
&(10,98,108),(48,25,73),(43,34,77),(2,20,22),(23,61,84),(101,4,105),(81,7,88),(3,65,68),\\
&(31,62,93),(16,64,80),(44,47,91),(56,53,109),(15,51,66),(11,19,30),(42,36,78),(21,74,95),\\
&(39,71,110),(32,54,86),(27,69,96),(63,40,103),(76,9,85),(46,26,72),(41,58,99),(33,37,70),\\
&(52,38,90),(13,87,100),(82,24,106),(14,97,111),(29,60,89),(57,35,92),(79,28,107),(45,59,104)\\
\hline 
\(n=123\) & 
2,14,3,5,1,11,13,4,6,16,64,91,78,105,17\\
\cline{2-2}
\(x=18\)
&(58,45,103),(61,21,82),(25,93,118),(69,51,120),(52,47,99),(62,18,80),(46,43,89),(34,40,74),\\
&(19,90,109),(22,88,110),(68,53,121),(65,54,119),(49,35,84),(66,38,104),(42,73,115),(86,31,117),\\
&(39,59,98),(9,63,72),(67,33,100),(28,94,122),(76,7,83),(75,48,123),(12,8,20),(41,70,111),\\
&(71,24,95),(97,15,112),(60,36,96),(56,50,106),(27,81,108),(23,32,55),(79,37,116),(29,85,114),\\
&(57,44,101),(10,92,102),(26,87,113),(77,30,107)\\
\hline 
\(n=135\) & 
29,10,63,92,7,28,57,70,99,120,49,116,59,126,127\\
\cline{2-2}
\(x=20\)
&(54,61,115),(129,4,133),(32,82,114),(104,19,123),(84,12,96),(11,83,94),(17,88,105),(20,18,38),\\
&(103,22,125),(52,46,98),(15,106,121),(33,69,102),(48,71,119),(74,16,90),(117,14,131),(47,44,91),\\
&(112,6,118),(5,95,100),(58,2,60),(8,85,93),(43,36,79),(41,35,76),(87,37,124),(30,81,111),\\
&(1,108,109),(77,9,86),(25,40,65),(64,66,130),(3,110,113),(51,21,72),(23,27,50),(80,42,122),\\
&(67,68,135),(53,75,128),(13,26,39),(55,34,89),(24,73,97),(62,45,107),(56,78,134),(31,101,132)\\
\hline 
\end{tabular}

==> tables/order-15-odd-labelings.tex <==
\begin{tabular}{| c | c |}
\hline
\(n\) and \(x\) & Base Labeling and Difference Triples\\
\hline
\(n=21\) & 
2,7,10,12,4,3,5,14,16,15,6,11,13,18,19\\
\cline{2-2}
\(x=1\)
&(9,8,17),(20,1,21)\\
\hline 
\(n=33\) & 
17,7,9,26,1,5,22,10,27,31,21,11,28,18,32\\
\cline{2-2}
\(x=3\)
&(12,2,14),(3,16,19),(6,24,30),(20,13,33),(4,25,29),(15,8,23)\\
\hline 
\(n=45\) & 
11,29,10,21,7,16,27,17,28,37,2,12,31,41,44\\
\cline{2-2}
\(x=5\)
&(4,39,43),(20,5,25),(34,1,35),(9,6,15),(33,3,36),(8,30,38),(14,26,40),(18,24,42),\\
&(22,23,45),(13,19,32)\\
\hline 
\(n=57\) & 
24,3,10,34,12,6,30,22,46,40,36,20,39,23,52\\
\cline{2-2}
\(x=7\)
&(25,1,26),(14,19,33),(17,28,45),(16,21,37),(31,18,49),(32,11,43),(15,29,44),(38,13,51),\\
&(48,7,55),(9,41,50),(42,5,47),(27,8,35),(53,4,57),(54,2,56)\\
\hline 
\(n=69\) & 
16,19,14,30,17,22,38,31,47,52,36,9,55,28,69\\
\cline{2-2}
\(x=9\)
&(23,35,58),(10,43,53),(24,20,44),(4,11,15),(2,46,48),(34,29,63),(33,27,60),(18,21,39),\\
&(62,5,67),(32,25,57),(40,26,66),(50,1,51),(7,61,68),(13,41,54),(8,56,64),(12,37,49),\\
&(3,42,45),(6,59,65)\\
\hline 
\(n=81\) & 
4,27,37,41,5,7,11,42,46,48,22,47,49,74,53\\
\cline{2-2}
\(x=11\)
&(21,18,39),(3,33,36),(8,70,78),(45,23,68),(61,16,77),(2,57,59),(31,19,50),(72,1,73),\\
&(40,29,69),(35,32,67),(13,63,76),(20,34,54),(10,52,62),(60,6,66),(44,12,56),(55,25,80),\\
&(15,9,24),(51,30,81),(26,38,64),(58,17,75),(65,14,79),(43,28,71)\\
\hline 
\(n=93\) & 
5,43,14,19,2,51,56,16,21,70,45,15,88,58,72\\
\cline{2-2}
\(x=13\)
&(54,22,76),(52,28,80),(20,48,68),(13,25,38),(24,40,64),(27,57,84),(31,47,78),(6,81,87),\\
&(71,8,79),(53,33,86),(10,75,85),(46,44,90),(18,12,30),(7,62,69),(36,41,77),(23,50,73),\\
&(1,66,67),(55,37,92),(35,26,61),(65,17,82),(74,9,83),(11,49,60),(29,34,63),(39,3,42),\\
&(59,32,91),(89,4,93)\\
\hline 
\(n=105\) & 
2,69,3,5,60,11,13,63,65,16,35,29,104,98,76\\
\cline{2-2}
\(x=15\)
&(28,34,62),(27,23,50),(43,39,82),(12,44,56),(30,6,36),(32,42,74),(9,94,103),(70,26,96),\\
&(14,58,72),(19,81,100),(31,52,83),(48,40,88),(10,80,90),(25,61,86),(33,59,92),(8,89,97),\\
&(38,55,93),(79,20,99),(51,15,66),(37,47,84),(17,68,85),(22,45,67),(18,73,91),(21,54,75),\\
&(71,24,95),(49,53,102),(77,1,78),(101,4,105),(7,57,64),(41,46,87)\\
\hline 
\(n=117\) & 
5,11,46,51,6,26,31,52,57,77,69,103,80,114,83\\
\cline{2-2}
\(x=17\)
&(20,50,70),(38,23,61),(34,68,102),(13,35,48),(81,15,96),(7,84,91),(8,10,18),(9,99,108),\\
&(67,28,95),(21,45,66),(1,58,59),(43,36,79),(56,19,75),(65,42,107),(63,37,100),(24,86,110),\\
&(30,71,101),(22,93,115),(53,25,78),(94,4,98),(29,87,116),(16,44,60),(104,2,106),(47,64,111),\\
&(33,49,82),(85,12,97),(89,3,92),(55,54,109),(72,40,112),(14,62,76),(74,39,113),(88,17,105),\\
&(41,32,73),(90,27,117)\\
\hline 
\(n=129\) & 
30,21,52,82,32,11,41,84,114,93,45,62,66,83,125\\
\cline{2-2}
\(x=19\)
&(72,7,79),(33,65,98),(86,22,108),(5,115,120),(55,39,94),(61,38,99),(2,27,29),(51,18,69),\\
&(23,88,111),(77,44,121),(6,19,25),(76,46,122),(53,37,90),(101,3,104),(14,67,81),(64,49,113),\\
&(73,56,129),(17,63,80),(119,8,127),(74,43,117),(47,28,75),(97,26,123),(70,40,110),(24,36,60),\\
&(16,89,105),(57,59,116),(54,42,96),(48,78,126),(10,85,95),(87,31,118),(58,13,71),(4,124,128),\\
&(106,1,107),(34,68,102),(100,9,109),(15,35,50),(20,92,112),(91,12,103)\\
\hline 
\end{tabular}

==> tables/order-16-even-labelings.tex <==
\begin{tabular}{| c | c |}
\hline
\(n\) and \(x\) & Base Labeling and Difference Triples\\
\hline
\(n=28\) & 
2,5,4,7,6,8,15,17,20,22,12,11,23,16,28,18\\
\cline{2-2}
\(x=2\)
&(9,10,19),(21,3,24),(14,13,27),(25,1,26)\\
\hline 
\(n=40\) & 
3,5,19,26,7,10,17,20,22,25,11,8,27,30,32,34\\
\cline{2-2}
\(x=4\)
&(13,16,29),(1,38,39),(4,24,28),(14,23,37),(6,12,18),(9,31,40),(15,21,36),(2,33,35)\\
\hline 
\(n=52\) & 
18,2,4,23,1,19,15,33,17,35,41,20,34,45,36,43\\
\cline{2-2}
\(x=6\)
&(40,6,46),(9,16,25),(29,21,50),(14,37,51),(5,7,12),(27,3,30),(32,10,42),(31,13,44),\\
&(26,22,48),(38,11,49),(28,24,52),(8,39,47)\\
\hline 
\(n=64\) & 
2,38,42,1,8,10,11,13,49,51,4,19,21,46,59,20\\
\cline{2-2}
\(x=8\)
&(29,34,63),(16,23,39),(33,22,55),(30,28,58),(41,15,56),(32,12,44),(37,27,64),(3,50,53),\\
&(31,17,48),(5,40,45),(35,25,60),(7,47,54),(14,43,57),(9,52,61),(18,6,24),(26,36,62)\\
\hline 
\(n=76\) & 
3,34,44,33,28,31,1,4,35,38,30,12,32,74,66,45\\
\cline{2-2}
\(x=10\)
&(36,40,76),(10,63,73),(16,54,70),(26,39,65),(19,48,67),(25,43,68),(29,46,75),(2,20,22),\\
&(53,9,62),(18,37,55),(41,17,58),(5,56,61),(24,23,47),(21,50,71),(52,7,59),(8,6,14),\\
&(49,11,60),(57,15,72),(51,13,64),(42,27,69)\\
\hline 
\(n=88\) & 
3,9,37,17,71,74,2,5,11,14,38,40,76,75,85,57\\
\cline{2-2}
\(x=12\)
&(20,12,32),(13,64,77),(53,34,87),(55,26,81),(72,1,73),(43,35,78),(18,70,88),(4,47,51),\\
&(58,7,65),(8,44,52),(66,16,82),(19,61,80),(45,41,86),(31,15,46),(39,24,63),(42,25,67),\\
&(33,21,54),(22,28,50),(60,23,83),(29,27,56),(36,48,84),(62,6,68),(49,30,79),(10,59,69)\\
\hline 
\(n=100\) & 
36,6,30,29,23,59,4,40,10,46,24,68,63,54,69,97\\
\cline{2-2}
\(x=14\)
&(79,7,86),(22,50,72),(28,47,75),(38,51,89),(39,3,42),(76,2,78),(19,26,45),(20,73,93),\\
&(33,15,48),(12,88,100),(60,17,77),(13,67,80),(5,57,62),(84,14,98),(35,18,53),(37,27,64),\\
&(66,25,91),(32,49,81),(8,82,90),(34,58,92),(11,74,85),(56,43,99),(16,71,87),(44,21,65),\\
&(41,55,96),(1,94,95),(31,52,83),(61,9,70)\\
\hline 
\(n=112\) & 
22,38,32,39,31,53,21,43,59,81,29,62,74,61,112,101\\
\cline{2-2}
\(x=16\)
&(65,19,84),(34,41,75),(71,17,88),(25,26,51),(23,82,105),(33,36,69),(57,54,111),(44,20,64),\\
&(73,24,97),(49,28,77),(72,11,83),(55,30,85),(47,46,93),(35,13,48),(12,58,70),(63,45,108),\\
&(40,56,96),(52,15,67),(4,103,107),(9,80,89),(76,14,90),(42,50,92),(18,68,86),(78,16,94),\\
&(91,7,98),(27,10,37),(60,6,66),(95,5,100),(99,3,102),(104,2,106),(8,79,87),(109,1,110)\\
\hline 
\(n=124\) & 
51,15,65,1,27,78,28,79,43,94,42,29,106,107,121,30\\
\cline{2-2}
\(x=18\)
&(66,34,100),(8,114,122),(14,54,68),(97,18,115),(92,25,117),(9,73,82),(33,38,71),(98,22,120),\\
&(89,10,99),(55,53,108),(56,37,93),(109,2,111),(58,45,103),(31,52,83),(77,11,88),(4,72,76),\\
&(57,47,104),(39,36,75),(19,86,105),(63,24,87),(61,49,110),(7,60,67),(44,41,85),(16,64,80),\\
&(70,46,116),(62,40,102),(21,74,95),(5,118,123),(50,69,119),(32,59,91),(35,13,48),(17,96,113),\\
&(112,12,124),(81,20,101),(6,84,90),(23,3,26)\\
\hline 
\(n=136\) & 
51,10,40,105,16,67,13,64,23,74,22,20,80,62,90,125\\
\cline{2-2}
\(x=20\)
&(70,63,133),(19,68,87),(109,17,126),(66,44,110),(54,25,79),(11,107,118),(32,61,93),(65,58,123),\\
&(92,24,116),(46,85,131),(53,49,102),(97,38,135),(39,37,76),(43,48,91),(34,100,134),(1,113,114),\\
&(98,29,127),(27,57,84),(30,82,112),(101,35,136),(4,117,121),(47,41,88),(21,111,132),(42,73,115),\\
&(45,75,120),(12,94,106),(3,78,81),(6,124,130),(60,59,119),(99,9,108),(89,14,103),(33,36,69),\\
&(8,96,104),(7,122,129),(56,72,128),(5,50,55),(31,52,83),(77,18,95),(71,15,86),(2,26,28)\\
\hline 
\end{tabular}

==> tables/order-18-even-labelings.tex <==
\begin{tabular}{| c | c |}
\hline
\(n\) and \(x\) & Base Labeling and Difference Triples\\
\hline
\(n=30\) & 
4,3,15,21,13,24,1,28,19,16,2,6,5,9,29,20,26,30\\
\cline{2-2}
\(x=2\)
&(10,17,27),(14,8,22),(11,12,23),(7,18,25)\\
\hline 
\(n=42\) & 
14,19,23,1,13,20,2,36,33,25,8,22,27,41,38,35,28,42\\
\cline{2-2}
\(x=4\)
&(24,15,39),(12,17,29),(31,3,34),(7,11,18),(26,6,32),(21,16,37),(10,30,40),(4,5,9)\\
\hline 
\(n=54\) & 
1,35,10,3,7,38,9,17,23,19,12,13,47,48,26,32,50,51\\
\cline{2-2}
\(x=6\)
&(2,27,29),(5,25,30),(39,14,53),(21,24,45),(20,22,42),(28,15,43),(31,18,49),(6,34,40),\\
&(37,4,41),(33,11,44),(16,36,52),(8,46,54)\\
\hline 
\(n=66\) & 
6,32,47,25,3,57,11,50,7,58,2,8,34,40,61,18,59,65\\
\cline{2-2}
\(x=8\)
&(52,12,64),(45,10,55),(29,15,44),(30,24,54),(26,37,63),(13,35,48),(14,46,60),(21,41,62),\\
&(42,9,51),(5,31,36),(22,17,39),(33,23,56),(16,27,43),(4,49,53),(1,19,20),(28,38,66)\\
\hline 
\(n=78\) & 
26,4,24,7,41,11,9,65,13,33,10,36,14,40,74,22,21,47\\
\cline{2-2}
\(x=10\)
&(5,55,60),(39,31,70),(64,3,67),(19,30,49),(48,23,71),(58,1,59),(46,27,73),(53,8,61),\\
&(12,45,57),(25,50,75),(2,76,78),(38,28,66),(20,32,52),(37,6,43),(42,35,77),(18,44,62),\\
&(29,34,63),(56,16,72),(51,17,68),(15,54,69)\\
\hline 
\(n=90\) & 
3,29,32,44,25,73,33,57,42,65,5,8,34,37,90,75,78,81\\
\cline{2-2}
\(x=12\)
&(20,27,47),(11,43,54),(36,31,67),(45,18,63),(72,12,84),(35,4,39),(6,77,83),(30,49,79),\\
&(7,55,62),(69,16,85),(74,14,88),(10,58,68),(61,21,82),(50,9,59),(56,15,71),(1,86,87),\\
&(22,38,60),(2,17,19),(26,40,66),(28,52,80),(13,51,64),(46,24,70),(41,48,89),(23,53,76)\\
\hline 
\(n=102\) & 
10,17,13,36,9,53,77,22,12,90,31,41,48,58,99,89,84,94\\
\cline{2-2}
\(x=14\)
&(45,47,92),(43,16,59),(62,34,96),(27,75,102),(33,64,97),(1,28,29),(37,20,57),(49,52,101),\\
&(26,61,87),(60,19,79),(72,23,95),(25,42,67),(66,15,81),(69,14,83),(76,2,78),(18,73,91),\\
&(82,3,85),(80,8,88),(35,5,40),(93,7,100),(50,6,56),(24,46,70),(51,4,55),(32,39,71),\\
&(63,11,74),(44,54,98),(30,38,68),(65,21,86)\\
\hline 
\(n=114\) & 
10,75,41,7,35,82,29,76,27,70,16,26,91,101,105,56,98,108\\
\cline{2-2}
\(x=16\)
&(94,19,113),(21,30,51),(90,9,99),(12,52,64),(65,46,111),(86,24,110),(22,61,83),(66,43,109),\\
&(62,11,73),(69,31,100),(17,28,45),(25,87,112),(15,39,54),(14,88,102),(50,13,63),(60,32,92),\\
&(58,37,95),(23,36,59),(49,44,93),(5,48,53),(1,96,97),(4,103,107),(2,55,57),(42,47,89),\\
&(72,34,106),(18,67,85),(81,33,114),(68,6,74),(38,40,78),(71,8,79),(84,20,104),(77,3,80)\\
\hline 
\(n=126\) & 
41,18,94,12,19,30,8,113,79,102,51,92,69,110,121,87,81,122\\
\cline{2-2}
\(x=18\)
&(60,46,106),(72,23,95),(45,74,119),(53,62,115),(11,66,77),(38,35,73),(14,20,34),(15,29,44),\\
&(93,10,103),(61,63,124),(96,24,120),(58,26,84),(27,5,32),(17,54,71),(108,1,109),(55,50,105),\\
&(13,112,125),(47,52,99),(65,2,67),(83,28,111),(49,68,117),(33,64,97),(37,39,76),(43,80,123),\\
&(42,40,82),(9,89,98),(90,36,126),(75,25,100),(70,31,101),(114,4,118),(7,78,85),(57,59,116),\\
&(56,48,104),(6,16,22),(3,88,91),(21,86,107)\\
\hline 
\(n=138\) & 
62,13,92,26,29,39,2,121,21,94,7,69,20,82,123,23,46,108\\
\cline{2-2}
\(x=20\)
&(5,110,115),(52,22,74),(66,31,97),(11,107,118),(122,14,136),(91,18,109),(6,106,112),(67,36,103),\\
&(65,24,89),(45,40,85),(10,68,78),(59,79,138),(56,42,98),(83,47,130),(25,102,127),(37,1,38),\\
&(57,60,117),(41,34,75),(93,27,120),(19,81,100),(33,28,61),(105,9,114),(90,44,134),(43,88,131),\\
&(16,119,135),(8,87,95),(3,96,99),(58,53,111),(4,129,133),(77,51,128),(17,63,80),(101,12,113),\\
&(64,73,137),(71,55,126),(84,48,132),(15,35,50),(30,86,116),(49,76,125),(70,54,124),(72,32,104)\\
\hline 
\end{tabular}

==> tables/order-32-even-labelings.tex <==
\begin{tabular}{| c | c |}
\hline
\(n\) and \(x\) & Base Labeling and Difference Triples\\
\hline
\(n=44\) & 
9,14,23,7,11,12,25,4,3,33,13,26,21,16,29,28,37,2,22,27,41,8,17,32,31,15,24,35,38,44,40,43\\
\cline{2-2}
\(x=2\)
&(20,10,30),(5,34,39),(1,18,19),(6,36,42)\\
\hline 
\(n=56\) & 
7,13,20,1,10,17,9,2,26,22,6,46,45,19,11,35,56,25,5,32,28,23,30,37,43,24,31,47,44,54,38,50\\
\cline{2-2}
\(x=4\)
&(33,18,51),(3,49,52),(34,14,48),(27,15,42),(41,12,53),(36,4,40),(39,16,55),(8,21,29)\\
\hline 
\(n=68\) & 
17,14,31,15,25,20,6,4,2,40,23,26,38,24,10,8,51,21,29,43,30,18,35,12,49,33,50,61,64,32,66,67\\
\cline{2-2}
\(x=6\)
&(5,52,57),(3,44,47),(11,48,59),(28,37,65),(53,7,60),(13,55,68),(34,22,56),(16,46,62),\\
&(19,39,58),(36,27,63),(9,45,54),(41,1,42)\\
\hline 
\(n=80\) & 
11,45,56,8,22,3,46,1,29,41,36,26,17,4,47,75,48,25,27,38,50,13,24,76,69,21,32,66,77,79,74,44\\
\cline{2-2}
\(x=8\)
&(64,7,71),(42,16,58),(37,23,60),(14,43,57),(34,19,53),(73,5,78),(6,62,68),(18,33,51),\\
&(2,70,72),(54,9,63),(65,15,80),(10,49,59),(31,30,61),(12,40,52),(20,35,55),(39,28,67)\\
\hline 
\(n=92\) & 
45,26,71,6,19,35,21,9,27,49,3,14,37,44,30,48,33,2,4,56,65,10,55,57,81,16,61,51,87,92,59,41\\
\cline{2-2}
\(x=10\)
&(11,68,79),(24,34,58),(18,28,46),(40,29,69),(5,85,90),(39,43,82),(12,62,74),(7,77,84),\\
&(22,54,76),(36,47,83),(66,20,86),(17,72,89),(31,60,91),(67,13,80),(63,1,64),(38,32,70),\\
&(52,23,75),(15,73,88),(8,42,50),(25,53,78)\\
\hline 
\(n=104\) & 
5,32,37,8,78,12,13,33,41,3,36,7,25,45,46,54,85,71,27,67,58,51,56,87,88,59,64,74,96,99,103,52\\
\cline{2-2}
\(x=12\)
&(4,30,34),(66,2,68),(70,9,79),(91,11,102),(29,60,89),(16,15,31),(6,55,61),(24,38,62),\\
&(35,42,77),(39,26,65),(22,76,98),(17,80,97),(1,47,48),(69,21,90),(50,44,94),(57,18,75),\\
&(28,72,100),(20,84,104),(10,73,83),(49,43,92),(63,23,86),(81,14,95),(40,53,93),(19,82,101)\\
\hline 
\(n=116\) & 
43,6,49,52,83,13,3,4,92,42,55,25,18,17,7,95,108,69,53,39,20,8,51,99,57,60,103,111,109,112,94,71\\
\cline{2-2}
\(x=14\)
&(56,22,78),(36,31,67),(54,37,91),(19,44,63),(30,84,114),(59,38,97),(35,27,62),(28,88,116),\\
&(46,34,80),(11,64,75),(26,79,105),(74,15,89),(58,29,87),(81,9,90),(41,72,113),(77,16,93),\\
&(65,50,115),(73,12,85),(32,66,98),(24,76,100),(96,5,101),(1,47,48),(10,23,33),(68,14,82),\\
&(70,40,110),(86,21,107),(102,2,104),(45,61,106)\\
\hline 
\(n=128\) & 
14,91,105,4,63,76,8,13,7,47,45,39,12,89,21,15,102,70,106,81,97,5,19,28,110,9,23,117,114,104,126,118\\
\cline{2-2}
\(x=16\)
&(51,65,116),(3,69,72),(90,18,108),(82,46,128),(35,20,55),(43,6,49),(29,37,66),(22,77,99),\\
&(96,16,112),(1,74,75),(40,85,125),(73,34,107),(36,48,84),(50,44,94),(27,88,115),(54,26,80),\\
&(92,11,103),(71,52,123),(78,17,95),(42,25,67),(68,59,127),(24,33,57),(2,98,100),(64,58,122),\\
&(62,31,93),(83,30,113),(32,87,119),(41,79,120),(86,38,124),(60,61,121),(53,56,109),(10,101,111)\\
\hline 
\end{tabular}

==> tables/order-5-even-labelings.tex <==
\begin{tabular}{| c | c |}
\hline
\(n\) and \(x\) & Base Labeling and Difference Triples\\
\hline
\(n=17\) & 
1,14,15,10,11\\
\cline{2-2}
\(x=2\)
&(6,7,13),(8,9,17),(12,4,16),(2,3,5)\\
\hline 
\(n=29\) & 
5,20,25,24,29\\
\cline{2-2}
\(x=4\)
&(13,15,28),(11,16,27),(10,8,18),(22,1,23),(2,12,14),(17,4,21),(6,3,9),(7,19,26)\\
\hline 
\(n=41\) & 
3,23,26,8,11\\
\cline{2-2}
\(x=6\)
&(6,27,33),(30,9,39),(14,18,32),(12,22,34),(28,1,29),(25,13,38),(31,5,36),(10,7,17),\\
&(24,16,40),(4,15,19),(35,2,37),(20,21,41)\\
\hline 
\(n=53\) & 
3,5,8,32,35\\
\cline{2-2}
\(x=8\)
&(33,18,51),(15,34,49),(13,31,44),(20,25,45),(26,27,53),(10,37,47),(23,29,52),(6,11,17),\\
&(14,16,30),(42,4,46),(9,12,21),(41,7,48),(1,39,40),(24,19,43),(2,36,38),(22,28,50)\\
\hline 
\(n=65\) & 
19,42,61,45,64\\
\cline{2-2}
\(x=10\)
&(39,23,62),(14,6,20),(21,22,43),(13,52,65),(16,18,34),(31,10,41),(2,38,40),(11,25,36),\\
&(29,26,55),(30,33,63),(7,37,44),(4,53,57),(46,8,54),(49,9,58),(5,12,17),(24,27,51),\\
&(28,32,60),(56,3,59),(47,1,48),(35,15,50)\\
\hline 
\(n=77\) & 
29,15,44,34,63\\
\cline{2-2}
\(x=12\)
&(7,50,57),(21,45,66),(26,47,73),(23,17,40),(25,24,49),(30,22,52),(38,27,65),(2,46,48),\\
&(10,6,16),(20,36,56),(28,33,61),(1,76,77),(32,3,35),(43,31,74),(54,14,68),(64,5,69),\\
&(58,9,67),(62,8,70),(37,18,55),(71,4,75),(39,12,51),(11,42,53),(59,13,72),(19,41,60)\\
\hline 
\(n=89\) & 
21,19,40,62,83\\
\cline{2-2}
\(x=14\)
&(22,43,65),(53,34,87),(30,59,89),(69,6,75),(35,28,63),(42,15,57),(10,61,71),(48,33,81),\\
&(66,20,86),(12,14,26),(27,58,85),(17,51,68),(38,18,56),(47,3,50),(31,24,55),(72,2,74),\\
&(49,11,60),(1,4,5),(64,9,73),(13,16,29),(46,32,78),(44,23,67),(76,8,84),(39,41,80),\\
&(52,36,88),(25,54,79),(7,70,77),(37,45,82)\\
\hline 
\(n=101\) & 
11,58,69,32,43\\
\cline{2-2}
\(x=16\)
&(5,50,55),(57,28,85),(77,7,84),(26,12,38),(59,6,65),(29,54,83),(45,2,47),(4,33,37),\\
&(72,25,97),(61,3,64),(24,44,68),(22,27,49),(51,39,90),(17,53,70),(31,67,98),(16,20,36),\\
&(30,71,101),(42,34,76),(19,80,99),(18,60,78),(75,13,88),(8,74,82),(10,63,73),(14,81,95),\\
&(92,1,93),(23,66,89),(9,87,96),(35,56,91),(46,40,86),(48,52,100),(41,21,62),(15,79,94)\\
\hline 
\(n=113\) & 
15,75,90,30,45\\
\cline{2-2}
\(x=18\)
&(14,72,86),(50,44,94),(32,28,60),(11,9,20),(36,68,104),(54,41,95),(43,53,96),(57,17,74),\\
&(37,63,100),(47,29,76),(48,49,97),(77,12,89),(19,83,102),(18,6,24),(82,10,92),(61,23,84),\\
&(78,21,99),(13,66,79),(64,42,106),(38,33,71),(56,51,107),(52,35,87),(16,85,101),(27,46,73),\\
&(22,59,81),(5,65,70),(40,58,98),(80,25,105),(55,7,62),(108,4,112),(34,69,103),(3,88,91),\\
&(111,2,113),(109,1,110),(8,31,39),(26,67,93)\\
\hline 
\(n=125\) & 
9,84,93,52,61\\
\cline{2-2}
\(x=20\)
&(46,4,50),(30,60,90),(12,65,77),(56,53,109),(59,39,98),(44,36,80),(25,100,125),(92,32,124),\\
&(11,99,110),(49,68,117),(96,24,120),(26,82,108),(33,1,34),(5,66,71),(28,91,119),(20,75,95),\\
&(79,27,106),(85,2,87),(86,17,103),(62,54,116),(22,83,105),(64,6,70),(8,10,18),(76,21,97),\\
&(16,41,57),(3,55,58),(40,7,47),(51,72,123),(102,19,121),(74,48,122),(35,78,113),(45,67,112),\\
&(13,101,114),(73,42,115),(38,69,107),(89,15,104),(14,29,43),(23,88,111),(81,37,118),(63,31,94)\\
\hline 
\(n=137\) & 
35,88,123,3,38\\
\cline{2-2}
\(x=22\)
&(57,55,112),(48,71,119),(30,106,136),(16,33,49),(109,15,124),(18,72,90),(32,98,130),(99,23,122),\\
&(76,56,132),(103,12,115),(66,68,134),(13,118,131),(46,37,83),(10,7,17),(40,70,110),(87,42,129),\\
&(9,54,63),(92,22,114),(58,27,85),(4,89,93),(102,25,127),(100,11,111),(6,91,97),(2,84,86),\\
&(69,59,128),(21,44,65),(29,50,79),(51,75,126),(101,34,135),(113,8,121),(47,5,52),(39,94,133),\\
&(24,96,120),(20,53,73),(116,1,117),(81,14,95),(43,82,125),(74,31,105),(77,60,137),(78,26,104),\\
&(45,62,107),(67,41,108),(36,28,64),(19,61,80)\\
\hline 
\end{tabular}

==> tables/order-5-odd-labelings.tex <==
\begin{tabular}{| c | c |}
\hline
\(n\) and \(x\) & Base Labeling and Difference Triples\\
\hline
\(n=11\) & 
4,7,11,6,10\\
\cline{2-2}
\(x=1\)
&(1,8,9),(2,3,5)\\
\hline 
\(n=23\) & 
6,2,8,11,17\\
\cline{2-2}
\(x=3\)
&(12,9,21),(3,13,16),(10,4,14),(19,1,20),(5,18,23),(7,15,22)\\
\hline 
\(n=35\) & 
18,2,20,10,28\\
\cline{2-2}
\(x=5\)
&(6,1,7),(30,4,34),(17,16,33),(8,27,35),(21,11,32),(13,12,25),(15,14,29),(9,22,31),\\
&(19,5,24),(3,23,26)\\
\hline 
\(n=47\) & 
6,39,45,34,40\\
\cline{2-2}
\(x=7\)
&(21,22,43),(23,4,27),(10,18,28),(3,35,38),(19,13,32),(2,7,9),(12,17,29),(25,1,26),\\
&(14,16,30),(24,20,44),(8,33,41),(31,15,46),(37,5,42),(36,11,47)\\
\hline 
\(n=59\) & 
10,38,48,43,53\\
\cline{2-2}
\(x=9\)
&(1,54,55),(39,20,59),(30,12,42),(2,16,18),(29,4,33),(44,8,52),(21,14,35),(28,17,45),\\
&(13,23,36),(24,26,50),(40,7,47),(3,34,37),(41,15,56),(22,5,27),(9,49,58),(46,11,57),\\
&(6,25,31),(32,19,51)\\
\hline 
\(n=71\) & 
44,21,65,4,48\\
\cline{2-2}
\(x=11\)
&(11,30,41),(50,10,60),(16,7,23),(5,26,31),(38,28,66),(29,17,46),(20,35,55),(56,3,59),\\
&(42,25,67),(19,51,70),(45,2,47),(14,57,71),(34,18,52),(9,54,63),(37,6,43),(36,22,58),\\
&(1,32,33),(53,15,68),(24,40,64),(49,13,62),(27,12,39),(8,61,69)\\
\hline 
\(n=83\) & 
48,23,71,21,69\\
\cline{2-2}
\(x=13\)
&(10,43,53),(59,17,76),(28,34,62),(16,29,45),(31,52,83),(41,14,55),(26,6,32),(2,37,39),\\
&(46,33,79),(61,5,66),(42,12,54),(25,15,40),(60,8,68),(20,38,58),(13,36,49),(27,51,78),\\
&(19,44,63),(18,57,75),(9,56,65),(3,64,67),(73,7,80),(70,4,74),(11,24,35),(1,81,82),\\
&(47,30,77),(50,22,72)\\
\hline 
\(n=95\) & 
18,75,93,34,52\\
\cline{2-2}
\(x=15\)
&(81,8,89),(4,44,48),(6,71,77),(53,38,91),(37,46,83),(55,24,79),(50,1,51),(13,57,70),\\
&(65,22,87),(36,3,39),(56,32,88),(40,54,94),(42,30,72),(49,29,78),(23,69,92),(21,63,84),\\
&(47,33,80),(45,41,86),(10,5,15),(17,43,60),(35,26,61),(19,76,95),(62,20,82),(31,59,90),\\
&(27,58,85),(7,67,74),(12,16,28),(11,14,25),(64,9,73),(2,66,68)\\
\hline 
\(n=107\) & 
2,57,59,41,43\\
\cline{2-2}
\(x=17\)
&(66,28,94),(88,15,103),(42,49,91),(24,78,102),(23,76,99),(92,13,105),(37,36,73),(52,46,98),\\
&(34,33,67),(35,50,85),(14,25,39),(68,3,71),(26,22,48),(74,10,84),(19,87,106),(40,30,70),\\
&(55,45,100),(8,72,80),(86,7,93),(4,58,62),(32,75,107),(16,47,63),(56,21,77),(12,5,17),\\
&(60,44,104),(27,38,65),(18,61,79),(29,54,83),(20,69,89),(81,9,90),(95,6,101),(1,96,97),\\
&(11,53,64),(51,31,82)\\
\hline 
\(n=119\) & 
34,24,58,70,104\\
\cline{2-2}
\(x=19\)
&(84,27,111),(52,56,108),(26,28,54),(4,2,6),(46,48,94),(17,57,74),(53,61,114),(76,33,109),\\
&(86,7,93),(5,62,67),(3,78,81),(90,13,103),(9,97,106),(30,80,110),(16,89,105),(39,59,98),\\
&(49,50,99),(18,83,101),(43,44,87),(19,23,42),(75,21,96),(95,12,107),(35,36,71),(1,112,113),\\
&(8,65,73),(79,40,119),(63,22,85),(68,32,100),(45,72,117),(60,55,115),(77,41,118),(64,38,102),\\
&(51,37,88),(66,25,91),(47,69,116),(15,14,29),(20,11,31),(10,82,92)\\
\hline 
\(n=131\) & 
4,113,117,71,75\\
\cline{2-2}
\(x=21\)
&(25,81,106),(29,83,112),(104,1,105),(49,82,131),(59,51,110),(69,60,129),(107,8,115),(2,48,50),\\
&(18,15,33),(73,27,100),(68,62,130),(57,52,109),(43,56,99),(93,10,103),(34,92,126),(45,80,125),\\
&(9,111,120),(20,96,116),(89,13,102),(31,64,95),(44,84,128),(28,63,91),(88,30,118),(26,11,37),\\
&(55,39,94),(16,19,35),(41,46,87),(54,32,86),(38,76,114),(67,12,79),(23,47,70),(61,40,101),\\
&(65,58,123),(42,36,78),(108,14,122),(5,85,90),(66,6,72),(97,22,119),(53,74,127),(7,17,24),\\
&(77,21,98),(121,3,124)\\
\hline 
\end{tabular}
